Evolutionary Stochastic Gradient Descent for Optimization of Deep Neural Networks

We propose a population-based Evolutionary Stochastic Gradient Descent (ESGD) framework for optimizing deep neural networks. ESGD combines SGD and gradient-free evolutionary algorithms as complementary algorithms in one framework in which the optimization alternates between the SGD step and evolution step to improve the average fitness of the population. With a back-off strategy in the SGD step and an elitist strategy in the evolution step, it guarantees that the best fitness in the population will never degrade. In addition, individuals in the population optimized with various SGD-based optimizers using distinct hyper-parameters in the SGD step are considered as competing species in a coevolution setting such that the complementarity of the optimizers is also taken into account. The effectiveness of ESGD is demonstrated across multiple applications including speech recognition, image recognition and language modeling, using networks with a variety of deep architectures.

==> cifar10_exp.tex <==
To evaluate ESGD for the image recognition, we choose CIFAR10 dataset and its corresponding ResNet model.  The CIFAR10 dataset contains a 50K image training-set and a 10K image test-set. Each image is a 32x32 3-channel color image. There are 10 evenly distributed classes. The ResNet model used in this paper is a 20-depth ResNet with a 64x10 linear layer in the end and cross-entropy as criterion. Batch-normalization is used. Note CIFAR10 does not have a validation-set, to be consistent with the training-set used in the literature, we do not split a validation dataset from the training dataset; instead, we evaluate fitness score over the entire training dataset. For the baseline training, we follow the recipes proposed in ~\cite{FB-ResNet}. The initial learning rate is set as 0.1, annealed 10x at the 81-st epoch and annealed by another 10x. Training finishes in 160 epochs. Nesterov momentum acceleration is adopted with a default momentum 0.9.  The baseline model accuracy is 8.34\%. Initially, we used a 80/20 SGD/Adam configuration in ESGD. While training loss was significantly improved, generalization became worse as we encountered the same Adam generalization problem on data-sets like CIFAR10, as reported in ~\cite{marginaladam, SWATS} . We found the best strategy is to use SGD as the sole optimizer and create diversity via randomizing SGD hyper-parameters. We record detailed experimental configuration in Appendix. Table~\ref{tab:cifar10_exp} shows that ESGD clearly outperforms baseline in both fitness score and model accuracy.

\begin{table}[htb]
\caption{Performance of ESGD on CIFAR-10.}
\label{tab:cifar10_exp}
\centering
\begin{tabular}{l|c|c|c|c} \hline
             &    \multicolumn{2}{c|}{loss}              &    \multicolumn{2}{c}{WER}         \\ \cline{2-5}
             &  $\theta_{1:\mu}$ &  $\theta_{1:\mu} - \theta_{15:\mu}$  &  $\theta_{1:\mu}$ &  $\theta_{1:\mu} - \theta_{15:\mu}$  \\ \hline\hline
  single baseline  &     0.0176     &     --                   &     8.34      &     --             \\ \hline
  population baseline  &     0.0151     &   [0.0151, \ \ 0.0164]   &     8.24      &  [7.90, \ \  8.69]  \\ \hline
    ESGD \textbackslash \ Evolution       &     0.0147     &   [0.0147, \ \ 0.0166]   &     8.49      &  [7.86, \ \  8.53]  \\ \hline
  ESGD        &     0.0142     &   [0.0142, \ \ 0.0159]   &     7.52      &  [7.43, \ \  8.10]  \\ \hline

\end{tabular}
\end{table}



